How to include a three-nucleon force into Faddeev equations for the 3N continuum: a new form

A new, more efficient approach to include a three nucleon force into three-nucleon continuum calculations is presented. Results obtained in the new and our old approach are compared both for elastic nucleon-deuteron scattering as well as for the breakup process. The advantages of the new scheme are discussed.

==> fig1.tex <==
\input pictex
\magnification=\magstep2
  % Makros \rotatedtext und \Ytext zum
  % (90-Grad gedrehten) Beschriften z.B. der y-Achse
  % !!!  Verwendet \specials von dvips  !!!
  %   \Ytext {<Text>}
  %   \rotatedtext <Winkel>, {<Text>}
  \def\turntext#1{\special{ps:currentpoint currentpoint translate
     #1 neg rotate neg exch neg exch translate}}
  \def\Ytext#1{\setbox0=\hbox{#1}\dimen0=\ht0 \advance\dimen0 by\dp0
     \hbox to\dimen0{\hss\vbox to\wd0{\vss
     \special{ps:gsave}\turntext{90}%
       \hbox to0pt{\hss\vbox to0pt{\vss\box0\vss}\hss}
     \special{ps:grestore}\vss}\hss}}
  \def\rotatedtext#1,#2{\special{ps:gsave}\turntext{#1}%
       \hbox to0pt{\hss\vbox to0pt{\vss\hbox{#2}\vss}\hss}%
     \special{ps:grestore}}

\hsize=18truecm
\phantom.
\hskip -2 true cm
 \beginpicture
\setcoordinatesystem units < 1. true cm,    1. true cm>
\setplotarea x from  0. to  18. , y from  0. to 8
\put {

 \beginpicture
\setcoordinatesystem units < 0.03333333 true cm,    15.6743 true cm>
\setplotarea x from      0.0000 to    180.0000 , y from     -0.0089 to      0.3739
%\put {$ C_{yy} $} [l] <10pt,0pt> at      0.000      0.15
\put {\Ytext{$ C_{yy} $}} [l] <-40pt,0pt> at      0.000      .1825
 \linethickness .8 pt
 \setplotsymbol ({\sevenrm .})
\axis bottom label {$\vartheta$ [deg]} ticks short numbered from      0.0000 to    180.0000 by         45. /
\axis top ticks short unlabeled from      0.0000 to    180.0000 by         45. /
\axis left ticks short numbered from        0.00 to        0.30 by        0.10 /
\axis right ticks short unlabeled from        0.00 to        0.30 by        0.10 /
 \setplotsymbol ({\fiverm .})
 \setsolid                                                   
 \plot
     0.0000     0.28140000
     2.5000     0.28150001
     5.0000     0.28169999
     7.5000     0.28220001
    10.0000     0.28279999
    12.5000     0.28360000
    15.0000     0.28450000
    17.5000     0.28560001
    20.0000     0.28680000
    22.5000     0.28799999
    25.0000     0.28929999
    27.5000     0.29069999
    30.0000     0.29200000
    32.5000     0.29330000
    35.0000     0.29449999
    37.5000     0.29560000
    40.0000     0.29650000
    42.5000     0.29719999
    45.0000     0.29769999
    47.5000     0.29780000
    50.0000     0.29750001
    52.5000     0.29679999
    55.0000     0.29560000
    57.5000     0.29380000
    60.0000     0.29139999
    62.5000     0.28830001
    65.0000     0.28450000
    67.5000     0.27980000
    70.0000     0.27430001
    72.5000     0.26769999
    75.0000     0.26019999
    77.5000     0.25150001
    80.0000     0.24160001
    82.5000     0.23060000
    85.0000     0.21820000
    87.5000     0.20440000
    90.0000     0.18920000
    92.5000     0.17260000
    95.0000     0.15459999
    97.5000     0.13510001
   100.0000     0.11450000
   102.5000     0.09302000
   105.0000     0.07125000
   107.5000     0.05015000
   110.0000     0.03120000
   112.5000     0.01644000
   115.0000     0.00850700
   117.5000     0.01022000
   120.0000     0.02386000
   122.5000     0.05007000
   125.0000     0.08701000
   127.5000     0.13050000
   130.0000     0.17550001
   132.5000     0.21720000
   135.0000     0.25279999
   137.5000     0.28099999
   140.0000     0.30219999
   142.5000     0.31729999
   145.0000     0.32740000
   147.5000     0.33370000
   150.0000     0.33719999
   152.5000     0.33860001
   155.0000     0.33870000
   157.5000     0.33790001
   160.0000     0.33660001
   162.5000     0.33500001
   165.0000     0.33329999
   167.5000     0.33160001
   170.0000     0.33019999
   172.5000     0.32900000
   175.0000     0.32810000
   177.5000     0.32749999
   180.0000     0.32730001
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <8pt, 4pt>                                  
 \plot
     0.0000     0.31720001
     2.5000     0.31729999
     5.0000     0.31760001
     7.5000     0.31810001
    10.0000     0.31880000
    12.5000     0.31959999
    15.0000     0.32069999
    17.5000     0.32179999
    20.0000     0.32310000
    22.5000     0.32449999
    25.0000     0.32600001
    27.5000     0.32749999
    30.0000     0.32900000
    32.5000     0.33039999
    35.0000     0.33180001
    37.5000     0.33309999
    40.0000     0.33419999
    42.5000     0.33510000
    45.0000     0.33559999
    47.5000     0.33590001
    50.0000     0.33579999
    52.5000     0.33520001
    55.0000     0.33410001
    57.5000     0.33239999
    60.0000     0.33010000
    62.5000     0.32699999
    65.0000     0.32310000
    67.5000     0.31840000
    70.0000     0.31279999
    72.5000     0.30610001
    75.0000     0.29840001
    77.5000     0.28950000
    80.0000     0.27939999
    82.5000     0.26800001
    85.0000     0.25529999
    87.5000     0.24110000
    90.0000     0.22550000
    92.5000     0.20850000
    95.0000     0.18990000
    97.5000     0.17000000
   100.0000     0.14880000
   102.5000     0.12680000
   105.0000     0.10450000
   107.5000     0.08295000
   110.0000     0.06375000
   112.5000     0.04909000
   115.0000     0.04176000
   117.5000     0.04473000
   120.0000     0.06025000
   122.5000     0.08863000
   125.0000     0.12740000
   127.5000     0.17180000
   130.0000     0.21619999
   132.5000     0.25610000
   135.0000     0.28889999
   137.5000     0.31400001
   140.0000     0.33190000
   142.5000     0.34390000
   145.0000     0.35120001
   147.5000     0.35510001
   150.0000     0.35650000
   152.5000     0.35620001
   155.0000     0.35479999
   157.5000     0.35270000
   160.0000     0.35040000
   162.5000     0.34790000
   165.0000     0.34549999
   167.5000     0.34330001
   170.0000     0.34140000
   172.5000     0.33980000
   175.0000     0.33870000
   177.5000     0.33800000
   180.0000     0.33780000
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <4pt, 4pt>                                  
 \plot
     0.0000     0.31690001
     2.5000     0.31700000
     5.0000     0.31729999
     7.5000     0.31779999
    10.0000     0.31850001
    12.5000     0.31940001
    15.0000     0.32040000
    17.5000     0.32159999
    20.0000     0.32280001
    22.5000     0.32420000
    25.0000     0.32570001
    27.5000     0.32720000
    30.0000     0.32870001
    32.5000     0.33010000
    35.0000     0.33149999
    37.5000     0.33280000
    40.0000     0.33390000
    42.5000     0.33480000
    45.0000     0.33530000
    47.5000     0.33559999
    50.0000     0.33550000
    52.5000     0.33489999
    55.0000     0.33379999
    57.5000     0.33210000
    60.0000     0.32969999
    62.5000     0.32670000
    65.0000     0.32280001
    67.5000     0.31810001
    70.0000     0.31240001
    72.5000     0.30579999
    75.0000     0.29800001
    77.5000     0.28909999
    80.0000     0.27900001
    82.5000     0.26769999
    85.0000     0.25490001
    87.5000     0.24079999
    90.0000     0.22520000
    92.5000     0.20810001
    95.0000     0.18960001
    97.5000     0.16960000
   100.0000     0.14839999
   102.5000     0.12639999
   105.0000     0.10410000
   107.5000     0.08259000
   110.0000     0.06340000
   112.5000     0.04873000
   115.0000     0.04140000
   117.5000     0.04436000
   120.0000     0.05988000
   122.5000     0.08825000
   125.0000     0.12700000
   127.5000     0.17150000
   130.0000     0.21590000
   132.5000     0.25580001
   135.0000     0.28870001
   137.5000     0.31380001
   140.0000     0.33170000
   142.5000     0.34369999
   145.0000     0.35110000
   147.5000     0.35499999
   150.0000     0.35640001
   152.5000     0.35609999
   155.0000     0.35470000
   157.5000     0.35270000
   160.0000     0.35030001
   162.5000     0.34779999
   165.0000     0.34540001
   167.5000     0.34320000
   170.0000     0.34130001
   172.5000     0.33980000
   175.0000     0.33870000
   177.5000     0.33800000
   180.0000     0.33780000
 /
 \endpicture
} [lt] at 0. 8.
\put {

 \beginpicture
\setcoordinatesystem units < 0.03333333 true cm,     8.0747 true cm>
\setplotarea x from      0.0000 to    180.0000 , y from      0.0656 to      0.8087
%\put {$ K_y^{x'z'}*10  $} [l] <10pt,0pt> at      0.0000      0.6
\put {\Ytext{$10\ K_y^{x'z'}  $}} [l] <-40pt,0pt> at      0.0000      0.43715
 \linethickness .8 pt
 \setplotsymbol ({\sevenrm .})
\axis bottom label {$\vartheta$ [deg]} ticks short numbered from      0.0000 to    180.0000 by         45. /
\axis top ticks short unlabeled from      0.0000 to    180.0000 by         45. /
\axis left ticks short numbered from        0.10 to        0.80 by        0.20 /
\axis right ticks short unlabeled from        0.10 to        0.80 by        0.20 /
 \setplotsymbol ({\fiverm .})
 \setsolid                                                   
 \plot
     0.0000     0.14030001
     2.5000     0.14050001
     5.0000     0.14129999
     7.5000     0.14260000
    10.0000     0.14430000
    12.5000     0.14650001
    15.0000     0.14919999
    17.5000     0.15230000
    20.0000     0.15590000
    22.5000     0.15979999
    25.0000     0.16410001
    27.5000     0.16880000
    30.0000     0.17370000
    32.5000     0.17890000
    35.0000     0.18430001
    37.5000     0.18979999
    40.0000     0.19549999
    42.5000     0.20130000
    45.0000     0.20700000
    47.5000     0.21269999
    50.0000     0.21830000
    52.5000     0.22360000
    55.0000     0.22870001
    57.5000     0.23350000
    60.0000     0.23780000
    62.5000     0.24159999
    65.0000     0.24470000
    67.5000     0.24710000
    70.0000     0.24870001
    72.5000     0.24930000
    75.0000     0.24879999
    77.5000     0.24710000
    80.0000     0.24410000
    82.5000     0.23970000
    85.0000     0.23379999
    87.5000     0.22620000
    90.0000     0.21689999
    92.5000     0.20590000
    95.0000     0.19309999
    97.5000     0.17880000
   100.0000     0.16310000
   102.5000     0.14670001
   105.0000     0.13050000
   107.5000     0.11570000
   110.0000     0.10450000
   112.5000     0.09939000
   115.0000     0.10360000
   117.5000     0.12020000
   120.0000     0.15109999
   122.5000     0.19589999
   125.0000     0.25110000
   127.5000     0.31050000
   130.0000     0.36729997
   132.5000     0.41630000
   135.0000     0.45460001
   137.5000     0.48190001
   140.0000     0.49910003
   142.5000     0.50819999
   145.0000     0.51100004
   147.5000     0.50919998
   150.0000     0.50440001
   152.5000     0.49759999
   155.0000     0.48960000
   157.5000     0.48110002
   160.0000     0.47270000
   162.5000     0.46460000
   165.0000     0.45719999
   167.5000     0.45060003
   170.0000     0.44499999
   172.5000     0.44059998
   175.0000     0.43740001
   177.5000     0.43540001
   180.0000     0.43480003
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <8pt, 4pt>                                  
 \plot
     0.0000     0.16710000
     2.5000     0.16729999
     5.0000     0.16800000
     7.5000     0.16920000
    10.0000     0.17090000
    12.5000     0.17300001
    15.0000     0.17559999
    17.5000     0.17859998
    20.0000     0.18210000
    22.5000     0.18590000
    25.0000     0.19000000
    27.5000     0.19450000
    30.0000     0.19929999
    32.5000     0.20439999
    35.0000     0.20980000
    37.5000     0.21530001
    40.0000     0.22100000
    42.5000     0.22679999
    45.0000     0.23269999
    47.5000     0.23860000
    50.0000     0.24460001
    52.5000     0.25040001
    55.0000     0.25620002
    57.5000     0.26190001
    60.0000     0.26729998
    62.5000     0.27249998
    65.0000     0.27739999
    67.5000     0.28189999
    70.0000     0.28600001
    72.5000     0.28970000
    75.0000     0.29290000
    77.5000     0.29549998
    80.0000     0.29769999
    82.5000     0.29949999
    85.0000     0.30080000
    87.5000     0.30180001
    90.0000     0.30270001
    92.5000     0.30360001
    95.0000     0.30510002
    97.5000     0.30750000
   100.0000     0.31160000
   102.5000     0.31849998
   105.0000     0.32940000
   107.5000     0.34590000
   110.0000     0.36990002
   112.5000     0.40340000
   115.0000     0.44739997
   117.5000     0.50180000
   120.0000     0.56370002
   122.5000     0.62760001
   125.0000     0.68610001
   127.5000     0.73229998
   130.0000     0.76200002
   132.5000     0.77490002
   135.0000     0.77329999
   137.5000     0.76090002
   140.0000     0.74140000
   142.5000     0.71799999
   145.0000     0.69270003
   147.5000     0.66720003
   150.0000     0.64249998
   152.5000     0.61909997
   155.0000     0.59740001
   157.5000     0.57760000
   160.0000     0.55989999
   162.5000     0.54420000
   165.0000     0.53070003
   167.5000     0.51920003
   170.0000     0.50989997
   172.5000     0.50260001
   175.0000     0.49740002
   177.5000     0.49430001
   180.0000     0.49329999
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <4pt, 4pt>                                  
 \plot
     0.0000     0.16700000
     2.5000     0.16729999
     5.0000     0.16800000
     7.5000     0.16920000
    10.0000     0.17090000
    12.5000     0.17300001
    15.0000     0.17559999
    17.5000     0.17859998
    20.0000     0.18200001
    22.5000     0.18580002
    25.0000     0.19000000
    27.5000     0.19450000
    30.0000     0.19920000
    32.5000     0.20430000
    35.0000     0.20960000
    37.5000     0.21509999
    40.0000     0.22080001
    42.5000     0.22660001
    45.0000     0.23250000
    47.5000     0.23840001
    50.0000     0.24429999
    52.5000     0.25020000
    55.0000     0.25590000
    57.5000     0.26150000
    60.0000     0.26690000
    62.5000     0.27210000
    65.0000     0.27689999
    67.5000     0.28140000
    70.0000     0.28540000
    72.5000     0.28900000
    75.0000     0.29209998
    77.5000     0.29479998
    80.0000     0.29690000
    82.5000     0.29850000
    85.0000     0.29980001
    87.5000     0.30070001
    90.0000     0.30149999
    92.5000     0.30230001
    95.0000     0.30360001
    97.5000     0.30590001
   100.0000     0.30990002
   102.5000     0.31660002
   105.0000     0.32729998
   107.5000     0.34359998
   110.0000     0.36740002
   112.5000     0.40059999
   115.0000     0.44440001
   117.5000     0.49860001
   120.0000     0.56040001
   122.5000     0.62430000
   125.0000     0.68290001
   127.5000     0.72930002
   130.0000     0.75929999
   132.5000     0.77249998
   135.0000     0.77129996
   137.5000     0.75919998
   140.0000     0.74000001
   142.5000     0.71680003
   145.0000     0.69169998
   147.5000     0.66630000
   150.0000     0.64170003
   152.5000     0.61840004
   155.0000     0.59679997
   157.5000     0.57709998
   160.0000     0.55939996
   162.5000     0.54369998
   165.0000     0.53020000
   167.5000     0.51879996
   170.0000     0.50949997
   172.5000     0.50220001
   175.0000     0.49710003
   177.5000     0.49400002
   180.0000     0.49290001
 /
 \endpicture
} [lt] at 9. 8.
 \endpicture


\vfill\end

==> fig2.tex <==
\input pictex
\magnification=\magstep2

  % Makros \rotatedtext und \Ytext zum
  % (90-Grad gedrehten) Beschriften z.B. der y-Achse
  % !!!  Verwendet \specials von dvips  !!!
  %   \Ytext {<Text>}
  %   \rotatedtext <Winkel>, {<Text>}
  \def\turntext#1{\special{ps:currentpoint currentpoint translate
     #1 neg rotate neg exch neg exch translate}}
  \def\Ytext#1{\setbox0=\hbox{#1}\dimen0=\ht0 \advance\dimen0 by\dp0
     \hbox to\dimen0{\hss\vbox to\wd0{\vss
     \special{ps:gsave}\turntext{90}%
       \hbox to0pt{\hss\vbox to0pt{\vss\box0\vss}\hss}
     \special{ps:grestore}\vss}\hss}}
  \def\rotatedtext#1,#2{\special{ps:gsave}\turntext{#1}%
       \hbox to0pt{\hss\vbox to0pt{\vss\hbox{#2}\vss}\hss}%
     \special{ps:grestore}}

\hsize=18truecm
\phantom.
\hskip -2 true cm
 \beginpicture
\setcoordinatesystem units < 1. true cm,    1. true cm>
\setplotarea x from  0. to  18. , y from  0. to 8
\put {

 \beginpicture
\setcoordinatesystem units < 0.12269938 true cm,     0.6609 true cm>
\setplotarea x from      0.0000 to     48.9000 , y from      3.5190 to     12.5977
%\put {$d^5\sigma\over d\Omega_1\ d\Omega_2\ dS$} [l] <5pt,0pt> at      0.0000     9.
%\put {$\left[ {\rm mb\over\rm MeV\ sr^2}\right]$} [l] <5pt,0pt> at      0.0000     7.5
\put {\Ytext{$d^5\sigma\over d\Omega_1\ d\Omega_2\ dS$ $\left[ {\rm mb\over\rm MeV\ sr^2}\right]$}} [l] <-40pt,0pt> at      0.0000     8.05835
 \linethickness .8 pt
 \setplotsymbol ({\sevenrm .})
\axis bottom label {$\vartheta$ [deg]} ticks short numbered from          0. to         40. by         20. /
\axis top ticks short unlabeled from          0. to         40. by         20. /
\axis left ticks short numbered from          5. to         12. by          3. /
\axis right ticks short unlabeled from          5. to         12. by          3. /
 \setplotsymbol ({\fiverm .})
 \setsolid                                                   
 \plot
     0.0000     4.25209999
     1.7000     4.25010014
     3.3000     4.23589993
     5.0000     4.20100021
     6.6000     4.15679979
     8.3000     4.13009977
     9.9000     4.14870024
    11.6000     4.23210001
    13.2000     4.39109993
    14.8000     4.62709999
    16.4000     4.93440008
    18.0000     5.30319977
    19.5000     5.72069979
    21.1000     6.17290020
    22.6000     6.64470005
    24.1000     7.12090015
    25.6000     7.58720016
    27.0000     8.03110027
    28.5000     8.44659996
    29.8000     8.82639980
    31.2000     9.16279984
    32.5000     9.44880009
    33.8000     9.67870045
    35.1000     9.84869957
    36.3000     9.95829964
    37.4000    10.00899982
    38.6000    10.00300026
    39.6000     9.94419956
    40.7000     9.83810043
    41.7000     9.68879986
    42.6000     9.50020027
    43.5000     9.27630043
    44.3000     9.02079964
    45.0000     8.73729992
    45.7000     8.43019962
    46.4000     8.13739967
    46.9000     7.84630013
    47.5000     7.56430006
    47.9000     7.29829979
    48.2000     7.05490017
    48.5000     6.84000015
    48.7000     6.65920019
    48.9000     6.51709986
    48.9000     6.41849995
    48.9000     6.36700010
    48.7000     6.36590004
    48.5000     6.41720009
    48.1000     6.52229977
    47.6000     6.68079996
    47.0000     6.89160013
    46.3000     7.15189981
    45.4000     7.45749998
    44.3000     7.80319977
    43.1000     8.18190002
    41.7000     8.58570004
    40.1000     9.00619984
    38.2000     9.43360043
    36.1000     9.85799980
    33.8000    10.26900005
    31.1000    10.65600014
    28.2000    11.00899982
    24.9000    11.32299995
    21.3000    11.59000015
    17.5000    11.80799961
    13.4000    11.97500038
     9.1000    12.09200001
     4.6000    12.16199970
     0.0000    12.18500042
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <8pt, 4pt>                                  
 \plot
     0.0000     3.93709993
     1.7000     3.95339990
     3.3000     3.99559999
     5.0000     4.02580023
     6.6000     4.00279999
     8.3000     3.94860005
     9.9000     3.93169999
    11.6000     3.99850011
    13.2000     4.15789986
    14.8000     4.41069984
    16.4000     4.74940014
    18.0000     5.15670013
    19.5000     5.60909986
    21.1000     6.08279991
    22.6000     6.56379986
    24.1000     7.04199982
    25.6000     7.50729990
    27.0000     7.95039988
    28.5000     8.36610031
    29.8000     8.74680042
    31.2000     9.08380032
    32.5000     9.36960030
    33.8000     9.59759998
    35.1000     9.76379967
    36.3000     9.86740017
    37.4000     9.90960026
    38.6000     9.89319992
    39.6000     9.82180023
    40.7000     9.70030022
    41.7000     9.53330040
    42.6000     9.32530022
    43.5000     9.08090019
    44.3000     8.80469990
    45.0000     8.50070000
    45.7000     8.17350006
    46.4000     7.85179996
    46.9000     7.52990007
    47.5000     7.21549988
    47.9000     6.91599989
    48.2000     6.63859987
    48.5000     6.38999987
    48.7000     6.17630005
    48.9000     6.00320005
    48.9000     5.87489986
    48.9000     5.79449987
    48.7000     5.76350021
    48.5000     5.78210020
    48.1000     5.84889984
    47.6000     5.96110010
    47.0000     6.11539984
    46.3000     6.30800009
    45.4000     6.53569984
    44.3000     6.79600000
    43.1000     7.08780003
    41.7000     7.41200018
    40.1000     7.76819992
    38.2000     8.14729977
    36.1000     8.53330040
    33.8000     8.90779972
    31.1000     9.25489998
    28.2000     9.56439972
    24.9000     9.83220005
    21.3000    10.05900002
    17.5000    10.24800014
    13.4000    10.39900017
     9.1000    10.51200008
     4.6000    10.58199978
     0.0000    10.60599995
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <4pt, 4pt>                                  
 \plot
     0.0000     3.93720007
     1.7000     3.95350003
     3.3000     3.99569988
     5.0000     4.02589989
     6.6000     4.00290012
     8.3000     3.94880009
     9.9000     3.93190002
    11.6000     3.99869990
    13.2000     4.15799999
    14.8000     4.41090012
    16.4000     4.74959993
    18.0000     5.15689993
    19.5000     5.60930014
    21.1000     6.08300018
    22.6000     6.56409979
    24.1000     7.04220009
    25.6000     7.50759983
    27.0000     7.95069981
    28.5000     8.36629963
    29.8000     8.74699974
    31.2000     9.08409977
    32.5000     9.36979961
    33.8000     9.59790039
    35.1000     9.76399994
    36.3000     9.86760044
    37.4000     9.90989971
    38.6000     9.89340019
    39.6000     9.82199955
    40.7000     9.70049953
    41.7000     9.53349972
    42.6000     9.32549953
    43.5000     9.08110046
    44.3000     8.80480003
    45.0000     8.50080013
    45.7000     8.17370033
    46.4000     7.85190010
    46.9000     7.53000021
    47.5000     7.21560001
    47.9000     6.91610003
    48.2000     6.63880014
    48.5000     6.39010000
    48.7000     6.17640018
    48.9000     6.00330019
    48.9000     5.87500000
    48.9000     5.79460001
    48.7000     5.76370001
    48.5000     5.78230000
    48.1000     5.84899998
    47.6000     5.96129990
    47.0000     6.11560011
    46.3000     6.30819988
    45.4000     6.53590012
    44.3000     6.79619980
    43.1000     7.08799982
    41.7000     7.41219997
    40.1000     7.76840019
    38.2000     8.14750004
    36.1000     8.53349972
    33.8000     8.90799999
    31.1000     9.25510025
    28.2000     9.56449986
    24.9000     9.83230019
    21.3000    10.05900002
    17.5000    10.24800014
    13.4000    10.39900017
     9.1000    10.51200008
     4.6000    10.58199978
     0.0000    10.60599995
 /
 \endpicture
} [lt] at 0. 8.
\put {

 \beginpicture
\setcoordinatesystem units < 0.12269938 true cm,     6.9939 true cm>
\setplotarea x from      0.0000 to     48.9000 , y from     -0.7079 to      0.1500
%\put {$A_y(d)*100$} [l] <10pt,0pt> at      15.  -0.1500
\put {\Ytext{$100\ A_y(d)$}} [l] <-50pt,0pt> at      0.  -0.27895
 \linethickness .8 pt
 \setplotsymbol ({\sevenrm .})
\axis bottom label {$\vartheta$ [deg]} ticks short numbered from          0. to         40. by         20. /
\axis top ticks short unlabeled from          0. to         40. by         20. /
\axis left ticks short numbered from       -0.70 to        0.10 by        0.20 /
\axis right ticks short unlabeled from       -0.70 to        0.10 by        0.20 /
 \setplotsymbol ({\fiverm .})
 \setsolid                                                   
 \plot
     0.0000     0.00000000
     1.7000    -0.00749710
     3.3000    -0.01702500
     5.0000    -0.03145500
     6.6000    -0.05459500
     8.3000    -0.09026300
     9.9000    -0.14070000
    11.6000    -0.20508999
    13.2000    -0.27914000
    14.8000    -0.35653001
    16.4000    -0.43088999
    18.0000    -0.49726000
    19.5000    -0.55264997
    21.1000    -0.59603000
    22.6000    -0.62778002
    24.1000    -0.64923000
    25.6000    -0.66222000
    27.0000    -0.66811001
    28.5000    -0.66888005
    29.8000    -0.66654003
    31.2000    -0.66200000
    32.5000    -0.65597999
    33.8000    -0.64899999
    35.1000    -0.64142001
    36.3000    -0.63392997
    37.4000    -0.62718999
    38.6000    -0.62162000
    39.6000    -0.61748999
    40.7000    -0.61486000
    41.7000    -0.61298001
    42.6000    -0.61080998
    43.5000    -0.60747999
    44.3000    -0.60232002
    45.0000    -0.59490001
    45.7000    -0.58526003
    46.4000    -0.57818002
    46.9000    -0.56920999
    47.5000    -0.55799001
    47.9000    -0.54409003
    48.2000    -0.52701002
    48.5000    -0.50625002
    48.7000    -0.48138002
    48.9000    -0.45212001
    48.9000    -0.41841999
    48.9000    -0.38060001
    48.7000    -0.33932000
    48.5000    -0.29565001
    48.1000    -0.25088999
    47.6000    -0.20649000
    47.0000    -0.16383000
    46.3000    -0.12414000
    45.4000    -0.08831400
    44.3000    -0.05695400
    43.1000    -0.03034300
    41.7000    -0.00850220
    40.1000     0.00875100
    38.2000     0.02173600
    36.1000     0.03085600
    33.8000     0.03655300
    31.1000     0.03927700
    28.2000     0.03946100
    24.9000     0.03751200
    21.3000     0.03380300
    17.5000     0.02867700
    13.4000     0.02244700
     9.1000     0.01540700
     4.6000     0.00783560
     0.0000     0.00000000
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <8pt, 4pt>                                  
 \plot
     0.0000     0.00000000
     1.7000    -0.01031600
     3.3000    -0.02436500
     5.0000    -0.04187000
     6.6000    -0.05864400
     8.3000    -0.07211800
     9.9000    -0.08718600
    11.6000    -0.11370000
    13.2000    -0.15386000
    14.8000    -0.20459999
    16.4000    -0.25972000
    18.0000    -0.31213999
    19.5000    -0.35589001
    21.1000    -0.38727000
    22.6000    -0.40680999
    24.1000    -0.41679001
    25.6000    -0.41990000
    27.0000    -0.41914001
    28.5000    -0.41605997
    29.8000    -0.41105002
    31.2000    -0.40485001
    32.5000    -0.39802998
    33.8000    -0.39094001
    35.1000    -0.38383001
    36.3000    -0.37726000
    37.4000    -0.37177998
    38.6000    -0.36774001
    39.6000    -0.36533001
    40.7000    -0.36456001
    41.7000    -0.36470002
    42.6000    -0.36471000
    43.5000    -0.36375001
    44.3000    -0.36112002
    45.0000    -0.35633999
    45.7000    -0.34933001
    46.4000    -0.34548000
    46.9000    -0.34000000
    47.5000    -0.33241999
    47.9000    -0.32216001
    48.2000    -0.30855998
    48.5000    -0.29095000
    48.7000    -0.26875001
    48.9000    -0.24174999
    48.9000    -0.21037999
    48.9000    -0.17544000
    48.7000    -0.13811000
    48.5000    -0.09983201
    48.1000    -0.06215000
    47.6000    -0.02655500
    47.0000     0.00573960
    46.3000     0.03389700
    45.4000     0.05747100
    44.3000     0.07635700
    43.1000     0.09069800
    41.7000     0.10090000
    40.1000     0.10749000
    38.2000     0.11081000
    36.1000     0.11102000
    33.8000     0.10832000
    31.1000     0.10292000
    28.2000     0.09509000
    24.9000     0.08515900
    21.3000     0.07346400
    17.5000     0.06035000
    13.4000     0.04615100
     9.1000     0.03117700
     4.6000     0.01570800
     0.0000     0.00000000
 /
 \setplotsymbol ({\fiverm .})
 \setdashpattern <4pt, 4pt>                                  
 \plot
     0.0000     0.00000000
     1.7000    -0.00980630
     3.3000    -0.02333100
     5.0000    -0.04028400
     6.6000    -0.05649400
     8.3000    -0.06946200
     9.9000    -0.08422400
    11.6000    -0.11074001
    13.2000    -0.15116000
    14.8000    -0.20232999
    16.4000    -0.25793001
    18.0000    -0.31081000
    19.5000    -0.35494998
    21.1000    -0.38662001
    22.6000    -0.40636998
    24.1000    -0.41650999
    25.6000    -0.41975001
    27.0000    -0.41903996
    28.5000    -0.41596001
    29.8000    -0.41095001
    31.2000    -0.40477002
    32.5000    -0.39797997
    33.8000    -0.39093000
    35.1000    -0.38387001
    36.3000    -0.37737000
    37.4000    -0.37195998
    38.6000    -0.36798000
    39.6000    -0.36561999
    40.7000    -0.36488000
    41.7000    -0.36500999
    42.6000    -0.36500999
    43.5000    -0.36401999
    44.3000    -0.36136001
    45.0000    -0.35655999
    45.7000    -0.34952998
    46.4000    -0.34566000
    46.9000    -0.34016001
    47.5000    -0.33257002
    47.9000    -0.32232001
    48.2000    -0.30875000
    48.5000    -0.29124999
    48.7000    -0.26924998
    48.9000    -0.24258001
    48.9000    -0.21165000
    48.9000    -0.17724000
    48.7000    -0.14049999
    48.5000    -0.10282000
    48.1000    -0.06571200
    47.6000    -0.03061200
    47.0000     0.00129950
    46.3000     0.02920800
    45.4000     0.05268000
    44.3000     0.07160800
    43.1000     0.08612900
    41.7000     0.09662100
    40.1000     0.10359000
    38.2000     0.10732000
    36.1000     0.10795999
    33.8000     0.10567001
    31.1000     0.10066000
    28.2000     0.09319299
    24.9000     0.08359200
    21.3000     0.07220000
    17.5000     0.05936700
    13.4000     0.04543000
     9.1000     0.03070400
     4.6000     0.01547400
     0.0000     0.00000000
 /
 \endpicture
} [lt] at 9. 8.
 \endpicture


\vfill\end
